eScope: A Fine-Grained Power Prediction Mechanism for Mobile Applications

Managing the limited energy on mobile platforms executing long-running, resource intensive streaming applications requires adapting an application's operators in response to their power consumption. For example, the frame refresh rate may be reduced if the rendering operation is consuming too much power. Currently, predicting an application's power consumption requires (1) building a device-specific power model for each hardware component, and (2) analyzing the application's code. This approach can be complicated and error-prone given the complexity of an application's logic and the hardware platforms with heterogeneous components that it may execute on. We propose eScope, an alternative method to directly estimate power consumption by each operator in an application. Specifically, eScope correlates an application's execution traces with its device-level energy draw. We implement eScope as a tool for Android platforms and evaluate it using workloads on several synthetic applications as well as two video stream analytics applications. Our evaluation suggests that eScope predicts an application's power use with 97% or better accuracy while incurring a compute time overhead of less than 3%.

==> Author.tex <==
\author{Atul Sandur}
\authornote{Both authors contributed equally to this research.}
\email{sandur2@illinois.edu}
% \orcid{1234-5678-9012}
\author{Dipayan Mukherjee}
\authornotemark[1]
\email{dipayan2@illinois.edu}
\affiliation{%
  \institution{University of Illinois, Urbana-Champaign}
  % \streetaddress{P.O. Box 1212}
  % \city{Dublin}
  % \state{Ohio}
  \country{USA}
  \postcode{61820}
}

\author{Kirill Mechitov}
\affiliation{%
  \institution{Embeddor Technologies}
  % \streetaddress{1 Th{\o}rv{\"a}ld Circle}
  % \city{Hekla}
  \country{USA}}
\email{kmechitov2@embedortech.com}

\author{Pratik Lahiri}
\affiliation{%
  \institution{University of Illinois, Urbana-Champaign}
  % \city{Rocquencourt}
  \country{USA}
}
\email{plahiri2@illinois.edu}

\author{Gul Agha}
\affiliation{%
 \institution{University of Illinois, Urbana-Champaign}
 % \streetaddress{Rono-Hills}
 % \city{Doimukh}
 % \state{Arunachal Pradesh}
 \country{USA}}
 \email{agha@illinois.edu}

 \renewcommand{\shortauthors}{Sandur and Mukherjee, et al.}

==> format.tex <==
\AtBeginDocument{%
  \providecommand\BibTeX{{%
    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

\setcopyright{acmcopyright}
\copyrightyear{2023}
\acmYear{2023}
\acmDOI{XXXXXXX.XXXXXXX}

\acmConference[ACM SIGMETRICS '24]{ Proceedings of the Nineteenth European Conference on Computer Systems }{23-26 April 2024}{ Athens, Greece}
\acmPrice{15.00}
\acmISBN{978-1-4503-XXXX-X/18/06}

% \acmSubmissionID{268}
\renewcommand\footnotetextcopyrightpermission[1]{}
\settopmatter{printfolios=true,printacmref=false}
\settopmatter{printacmref=false} % REMOVE IN FINAL VERSION

